Can Large Language Models Help Experimental Design for Causal Discovery?

Designing proper experiments and selecting optimal intervention targets is a longstanding problem in scientific or causal discovery. Identifying the underlying causal structure from observational data alone is inherently difficult. Obtaining interventional data, on the other hand, is crucial to causal discovery, yet it is usually expensive and time-consuming to gather sufficient interventional data to facilitate causal discovery. Previous approaches commonly utilize uncertainty or gradient signals to determine the intervention targets. However, numerical-based approaches may yield suboptimal results due to the inaccurate estimation of the guiding signals at the beginning when with limited interventional data. In this work, we investigate a different approach, whether we can leverage Large Language Models (LLMs) to assist with the intervention targeting in causal discovery by making use of the rich world knowledge about the experimental design in LLMs. Specifically, we present Large Language Model Guided Intervention Targeting (LeGIT) -- a robust framework that effectively incorporates LLMs to augment existing numerical approaches for the intervention targeting in causal discovery. Across 4 realistic benchmark scales, LeGIT demonstrates significant improvements and robustness over existing methods and even surpasses humans, which demonstrates the usefulness of LLMs in assisting with experimental design for scientific discovery.

==> tables/LowData.tex <==
% \begin{table*}[h!]\small\centering
% \caption{SHD with Std. , for real-world data.}
% \begin{tabular}{llllllll}
% \toprule
%       &                           AIT &                                             Random Choice & Round Robin & Degree Prob & GIT & \ours(missing)  \\
% \midrule
% alarm &   32.80 ± 8.42 &  34.80 ± 2.32 &       	25.00 ± 1.26     &     29.40 ± 4.67        &  19.60 ± 3.77 &  18.80 ± 1.33 \\
% asia &        &             &      1.40 ± 0.49        &           &     1.00 ± 0.00        &             \\
% child &     9.00 ± 3.29  &             &   3.40 ± 2.50        &   6.20 ± 2.48          &   2.80 ± 0.75   &  2.20 ± 1.30  \\
% insurance & 24.20 ± 7.47 & 23.40 ± 1.62 &       25.80 ± 2.93      &        17.40 ± 4.54     & 16.40 ± 3.14 & 15.8±3.11 \\
% \bottomrule
% \end{tabular}
% \label{app:tab:shd_real_world}
% \end{table*}

% \begin{table*}[h!]\centering
% \centering
% \caption{Average SHD with standard deviation (from 5 seeds) , for real-world data ($N = 1056$) .}
% \begin{tabular}{llllllll}
% \toprule
%                 & alarm               & asia                & child              & insurance          \\
% \midrule
% AIT             & 32.80 ± 8.42        &                    & 9.00 ± 3.29        & 24.20 ± 7.47       \\
% Random Choice   & 34.80 ± 2.32        &                    &                    & 23.40 ± 1.62       \\
% Round Robin     & 25.00 ± 1.26        & 1.40 ± 0.49        & 3.40 ± 2.50        & 25.80 ± 2.93       \\
% Degree Prob     & 29.40 ± 4.67        &                    & 6.20 ± 2.48        & 17.40 ± 4.54       \\
% GIT             & 19.60 ± 3.77        & 1.00 ± 0.00        & 2.80 ± 0.75        & 16.40 ± 3.14       \\
% \textbf{\ours}  & 18.80 ± 1.33        &                    & 2.20 ± 1.30        & 15.80 ± 3.11        \\
% \bottomrule
% \end{tabular}
% \label{app:tab:shd_real_world_transposed}
% \end{table*}


% \begin{table*}[h!]\centering
% \centering
% \caption{Average SHD with standard deviation (from 5 seeds), for real-world data ($N = 1056$).}
% \begin{tabular}{llllllll}
% \toprule
%                 & alarm               & asia                & child              & insurance          \\
% \midrule
% AIT             & 32.80 {\scriptsize ± 8.42}        &                    & 9.00 {\scriptsize ± 3.29}        & 24.20 {\scriptsize ± 7.47}       \\
% Random Choice   & 34.80 {\scriptsize ± 2.32}        &                    &                    & 23.40 {\scriptsize ± 1.62}       \\
% Round Robin     & 25.00 {\scriptsize ± 1.26}        & 1.40 {\scriptsize ± 0.49}        & 3.40 {\scriptsize ± 2.50}        & 25.80 {\scriptsize ± 2.93}       \\
% Degree Prob     & 29.40 {\scriptsize ± 4.67}        &                    & 6.20 {\scriptsize ± 2.48}        & 17.40 {\scriptsize ± 4.54}       \\
% GIT             & 19.60 {\scriptsize ± 3.77}        & 1.00 {\scriptsize ± 0.00}        & 2.80 {\scriptsize ± 0.75}        & 16.40 {\scriptsize ± 3.14}       \\
% \textbf{\ours}  & 18.80 {\scriptsize ± 1.33}        &                    & 2.20 {\scriptsize ± 1.30}        & 15.80 {\scriptsize ± 3.11}       \\
% \bottomrule
% \end{tabular}
% \label{app:tab:shd_real_world_transposed}
% \end{table*}
% \begin{table}[t]
% \caption{Average SHD with standard deviation (from 5 seeds) with Low Data, for real-world data (with $T = 33$ rounds, and a total number of intervention samples $N = 528$).}
% \centering\small\sc
% \begin{tabular}{llll}
% \toprule
% \textbf{Method}     & \textbf{alarm}               & \textbf{insurance}           & \textbf{child}              \\
% \midrule
% GIT                &  26.20 {\scriptsize ± 3.71}  &  22.40 {\scriptsize ± 3.72}   &    7.50 {\scriptsize ± 1.61}\\
% \midrule
% \rowcolor{SkyBlue!20} % Sets the background color of the last row to light sky blue
% \textbf{\ours} &  \textbf{26.00 {\scriptsize ± 5.25 }}  & \textbf{18.80 {\scriptsize ± 2.04}} &  \textbf{6.00 {\scriptsize ± 2.40}}  \\
% \bottomrule
% \end{tabular}
% \label{table:lowdata}
% \end{table}
%
% \begin{table}[h!]
% \caption{Average SHD with standard deviation (from 5 seeds) with Low Data, for real-world data ($T = 33$ rounds, $N = 528$).}
% \vspace{-1mm}
% \centering\small\sc
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lllll}
% \toprule
% \textbf{Method} & \textbf{Asia}                 & \textbf{Child}                & \textbf{Alarm}               & \textbf{Insurance}            \\
% \midrule
% GIT             & 1.80 {\scriptsize ± 0.75}    & 6.75 {\scriptsize ± 0.43}     & 27.20 {\scriptsize ± 4.71}   & 23.00 {\scriptsize ± 3.94}    \\
% \midrule
% \rowcolor{SkyBlue!20} 
% \textbf{\ours}         & \textbf{1.40 {\scriptsize ± 0.49} }   & \textbf{4.40  {\scriptsize ± 2.15} }    & \textbf{21.00  {\scriptsize ± 2.37}}   & \textbf{18.20 {\scriptsize ± 1.17}  }  \\
% \bottomrule
% \end{tabular}}
% \vspace{-3mm}
% \label{table:lowdata}
% \end{table}

\begin{table}[h!]
\caption{Average SHD with standard deviation (from 5 seeds) with Low Data, for real-world data ($T = 33$ rounds, $N = 528$).}
\vspace{-2mm}
\centering\small\sc
\resizebox{\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
\textbf{Method} & \textbf{Alarm}               & \textbf{Insurance}            & \textbf{Child}                & \textbf{Asia}                 \\
\midrule
GIT             & 27.20 {\scriptsize ± 4.71}   & 23.00 {\scriptsize ± 3.94}    & 6.75 {\scriptsize ± 0.43}     & 1.80 {\scriptsize ± 0.75}     \\
\midrule
\rowcolor{SkyBlue!20} 
\textbf{\ours}  & \textbf{21.00 {\scriptsize ± 2.37}} & \textbf{18.20 {\scriptsize ± 1.17}} & \textbf{4.40 {\scriptsize ± 2.15}}  & \textbf{1.40 {\scriptsize ± 0.49}}  \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\label{table:lowdata}
\end{table}

